Proof Reduction of Fair Stuttering Refinement of Asynchronous Systems and Applications

We present a series of definitions and theorems demonstrating how to reduce the requirements for proving system refinements ensuring containment of fair stuttering runs. A primary result of the work is the ability to reduce the requisite proofs on runs of a system of interacting state machines to a set of definitions and checks on single steps of a small number of state machines corresponding to the intuitive notions of freedom from starvation and deadlock. We further refine the definitions to afford an efficient explicit-state checking procedure in certain finite state cases. We demonstrate the proof reduction on versions of the Bakery Algorithm.

==> eptcsdata.tex <==
\providecommand{\firstpage}{78}
\providecommand{\publicationstatus}{Warren Hunt Jr.\ and Anna Slobodova (Eds.):\\
ACL2 Theorem Prover and its Applications\\
EPTCS 249, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.249.6}{10.4204/EPTCS.249.6}}

